NVCiM-PT: An NVCiM-assisted Prompt Tuning Framework for Edge LLMs

Large Language Models (LLMs) deployed on edge devices, known as edge LLMs, need to continuously fine-tune their model parameters from user-generated data under limited resource constraints. However, most existing learning methods are not applicable for edge LLMs because of their reliance on high resources and low learning capacity. Prompt tuning (PT) has recently emerged as an effective fine-tuning method for edge LLMs by only modifying a small portion of LLM parameters, but it suffers from user domain shifts, resulting in repetitive training and losing resource efficiency. Conventional techniques to address domain shift issues often involve complex neural networks and sophisticated training, which are incompatible for PT for edge LLMs. Therefore, an open research question is how to address domain shift issues for edge LLMs with limited resources. In this paper, we propose a prompt tuning framework for edge LLMs, exploiting the benefits offered by non-volatile computing-in-memory (NVCiM) architectures. We introduce a novel NVCiM-assisted PT framework, where we narrow down the core operations to matrix-matrix multiplication, which can then be accelerated by performing in-situ computation on NVCiM. To the best of our knowledge, this is the first work employing NVCiM to improve the edge LLM PT performance.

==> 1_intro_v0.tex <==
%%%%%% Version 1 %%%%%%

% large-scale AI models show promising abilities in causal inference. However, there are certain flaws in terms of personalization, data privacy, and offline situations. 

% On-device learning can be the solution to the above issues. However on-device learning can be difficult when large-scale models are deployed on resource-constrained devices. Existing solutions have certain issues: 1. A heavy workload even releases the amount of resources. 2. Only allow learning from a small amount of data. 3. Certain acceleration frameworks can be architecture or system-specific and lack extensibility.

% Prompt tuning can enable the large-scale AI model, which has an overwhelming size of weights, comprehensive reasoning capabilities, and highly resource-consuming in normal fine-tuning, to learn from user-generated data. What is prompt tuning? Add a soft prompt (a short tensor) to each prompt embedding, formalizing the input layer. Then expecting the output can be more user-preferred. Here we just need to train a small model to generate the corresponding appropriate soft prompt given a prompt embedding.

% Why prompt tuning can work? The larger the model, the more effective prompting can be, since such models have huge pre-learning knowledge, better alignment is more effective than parameter learning.

% Benefit: It only enables an extremely small piece of parameters to learn, no need to update layers in the transformer avoiding costly computation, and only update the input layers. Why this is important? We can enable a modularized large-scale edge AI system, where the model module can be highly integrated and specifically optimized to better fit the target device, and the tuning module can be co-designed to use additional/external resources. 

% Take an example, Mixtral-8*7B is an over 20 GB strong and heavy LLM, deploying it on an edge device is already very challenging, not to mention training it. However, prompt tuning can enable Mixtral-8*7B learning on edge devices.


%%%%%% Version 2 %%%%%%

Large Language Models (LLMs) are primarily deployed on centralized cloud platforms \cite{qin2024fl} (Cloud LLMs), raising significant concerns about user privacy and trustworthiness \cite{neel2023privacy}. These issues are particularly critical in domains such as healthcare \cite{Karabacak_Margetis_2023}, AI companionship \cite{xu2023large}, and personal assistance \cite{li2024personal}, where protecting user data and ensuring model reliability is crucial. To address these challenges, there is a shift towards developing personalized LLMs capable of generating tailored responses. These models are designed for deployment on edge devices (Edge LLMs), allowing users to retain control over their private data. By enabling local learning and adaptation, Edge LLMs offer a promising solution that balances powerful AI capabilities with enhanced privacy protection, potentially transforming how we interact with and benefit from language models.

To better customize for distinct users, edge LLMs must learn from user interactions. Under the constraint RAM and computational power on edge devices, the existing works mainly take two types of approaches to enable LLM learning on edge: retrieval-augmented generation (RAG) \cite{qin2024robust} and low-rank adaption (LoRA) \cite{qin2023enabling}. However, the recent studies on edge LLM \cite{qin2024empirical} found that RAG has limited improvement due to the small size of pre-trained parameters on edge LLM, while LoRA's high resource consumption can prevent it from learning a broad range of user-generated data. 

Prompt tuning \cite{lester2021power} (PT) as an alternative, having higher learning bounds than RAG with lower resource usage than LoRA, can become a good learning method for edge LLM. When an LLM is under prompt tuning, a prompt encoder will be concatenated into this model. The prompt encoder will initialize a matrix called soft prompt where \textit{n} vectors with length of LLM embedding size are assigned. Each vector can represent one token. Given a data sample \textbf{s}, the input embedding layer of LLM will convert the sample \textit{s} into embedding \textbf{Emb(s)}, which will be concatenated with the soft prompt under the setting of prompt tuning. The main idea of prompt tuning is to find a soft prompt to improve the LLM content generation ability by concatenating with every input embedding. 

\input{tables/prelim}

PT offers a parameter-efficient approach for aligning user inputs with pre-trained LLMs, typically adjusting less than 0.01\% of the model's parameters. However, its application to edge LLMs faces significant challenges. Despite the small parameter footprint, PT substantially impacts training and inference time due to the transformer's quadratic complexity \cite{shi2023dept}. Edge devices' constrained data buffers exacerbate domain shift issues as users switch between tasks, contrasting with cloud-based PT's ability to create versatile "one-for-all" (\textbf{One4All}) soft prompts from comprehensive datasets.

Interestingly, each unique input has an optimal \textbf{single} soft prompt \cite{nassereldine2024pi} that can significantly enhance LLM performance. Our comparative analysis of One4All and Single prompts across three edge LLMs and five datasets (detailed in the experimental section) reveals a striking performance gap. As shown in TABLE ~\ref{tab:one4all}, we compare three prompt tuning methods including Vanilla \cite{lester2021power}, DEPT \cite{shi2023dept}, and P-tuning v2 \cite{liu2021p}, which use one4all soft prompt with the approach where each data sample is paired with its optimal soft prompt. \dcheng{check the meaning of the previous sentence} The last approach can outperform the three traditional prompt tuning methods. This finding highlights the potential of single soft prompts to address domain shift and reduce resource usage in PT, offering a promising direction for edge LLM optimization.

While single soft prompts address domain shift and reduce prompt tuning (PT) resource usage, they introduce new challenges. Through preliminary studies, we find that the RAM usage for storing soft prompts can proportionally increase as the accumulation of soft prompts, potentially degrading system performance. Moreover, storing prompts on SSDs and transferring them to RAM introduces latency issues. The core function of single-prompt-based PT is essentially prompt retrieval, making Computing-in-Memory (CiM) architecture an ideal solution. CiM enables massive parallel processing within the memory array, minimizing data movement through in-situ access and enhancing throughput. Furthermore, integrating non-volatile memory (NVM) devices such as phase-change memories (PCMs), resistive RAMs (RRAMs), and ferroelectric FETs (FeFETs) allows CiM (NVCiM) to surpass conventional MOSFET-based designs in energy efficiency \cite{chen2016eyeriss}. \dcheng{Combinig single soft prompts and CiM }This approach effectively addresses the memory-intensive nature of single soft prompts while optimizing retrieval and processing efficiency.

\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/vir_token_size.pdf}
    \caption{Increasing memory size}
    \label{fig:virtual_token_size}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/soft_prompt_time.pdf}
    \caption{Increasing data moving time}
    \label{fig:soft_prompt_time}
  \end{subfigure}
  \caption{Resource by the storing soft prompt and data moving. 
  }
  \label{fig:combined_analysis}
\end{figure}

While NVCiM offers potential benefits, its implementation in PT faces significant challenges. NVCiM operations are vulnerable to various noise sources, including electronic noise (thermal, shot, and flicker), device-to-device variability, and line noise from supporting circuitry \cite{yan2024compute}. These factors can significantly degrade computations, especially in high-precision tasks where signal levels approach the noise floor. Moreover, the fixed dimensions of typical NVCiM arrays (e.g., 64x64) often mismatch with LLM embedding shapes (e.g., 100x2048 in FP32 precision). Consequently, trained soft prompts must be encoded to fit NVCiM array sizes while contending with device noise, potentially compromising PT performance when utilizing NVCiM-retrieved soft prompts. These challenges underscore the need for sophisticated encoding and noise-mitigation strategies in NVCiM-based PT systems.

In this paper, we propose a \rqin{tiny prompt tuning framework based on co-design of edge and NVCiM}. On edge, we design a data selection method to reduce the training workload. On NVCiM, we design a heuristic search algorithm to retrieve the appropriate stored soft prompt to match the input embedding. To promote the edge and NVCiM collaboration, we introduce a noise-adaptable prompt tuning method on the edge. \rqin{[This part need to be elaborated a little bit]}

The main contributions of this work can be summarized into three points.
\begin{itemize}[itemsep=0em]
    \item We first extend the one-for-all-based prompt tuning into optimal single soft prompt retrieval-based prompt tuning, which can only be implemented via emerging technologies like NVCiM.
    \item We introduce a co-design mode between normal edge devices and NVCiM, where each part can take its advantageous functionality and collaborate to obtain the best performance.
    \item \rqin{Through our experiments, we demonstrate ...}
\end{itemize}

\rqin{By Zheyu: embedding and soft prompt, how they connect each other, need to make this as a contribution or some explanation. Why using embedding can find the appropriate soft prompt.}





==> 2_related_v0.tex <==

\subsection{CiM Architectures and their NVMs}

% This section might follow this logic: 

% CiM architecture and functionality (function level, no need to go to circuit details) 
% -> Advantages of NVM-based CiM (e.g. in-memory, reduced data movement, NVM-storage, save energy, etc)
% -> However, device variations may destroy the functionality of NVM-based CiM architecture 
% -> briefly explain different sources of variations (don't talk about device defecting, which is another story
% -> In this paper, we investigate the impact of device variations and mitigate their impacts via HW-SW co-design.
% -> We use RRAM and FeFET-based CiM as two proxies to illustrate the performance of the proposed framework.  

% Maybe you can combine the related work of {CiM/device variations/exsiting noise mitigation methods} into one subsection. Then use another subsection to introduce LLM-related background.

In NVCiM's memory array, soft prompts and input embeddings are stored as matrices in NVM cells, such as PCMs, RRAMs, and FeFETs, at the intersections of vertical and horizontal lines. Operations within the memory array occur in the analog domain, leveraging physical properties directly. However, essential functions like shift-and-add for multiple bits and sorting to find top-k ranked values are performed in the digital domain. Digital-to-analog and analog-to-digital converters (DACs and ADCs) facilitate communication between these components.
%CiM architecture can conduct matrix-vector multiplication directly in memory, which can efficiently reduce the data movement overhead. 

NVCiM arrays are subject to various sources of variations and noise, primarily spatial and temporal variations. Spatial variations result from fabrication defects and exhibit both local and global correlations. FeFET devices also experience temporal variations due to stochastic memory switching and aging, causing conductance fluctuations when programmed at different times. These temporal variations are typically independent across devices and unrelated to the programmed value.

This work focuses on the impact of temporal variations in the programming process on DNN performance. Temporal variation causes the programmed resistance of a device to deviate from its expected value. The proposed framework can be extended to address other sources of variations with modifications.

Measurement results~\cite{yan2022swim, yan2021uncertainty} indicate that noise on DNN weights caused by device variations can be modeled as Gaussian noise with zero mean, each with a standard deviation associated with the weight value. This is represented by:

{\scriptsize
\begin{equation}\label{eq:dev_var}
    \mathbf{v} = \mathbf{v_0} + \Delta\mathbf{v}, \Delta\mathbf{v}\sim\mathcal{N}(0,\sigma_v)
\end{equation}
}
where $\mathbf{v}$ is the actual embedding deployed on the accelerators, $\mathbf{v_0}$ is the target embedding value, and $\sigma_v$ is experimentally measured. We have compiled measurement results from RRAM and FeFET devices, with specific values shown in TABLE ~\ref{tab:var}.

\begin{figure*}[t!]
  \centering
  \includegraphics[trim=0 392 284 0, clip, width=1.\linewidth]{figures/method_Long.pdf}
  \caption{Overview of our proposed NV\textbf{C}iM-based \textbf{P}rompt Tuning framework (\textbf{CP-tuning}). By co-design, it can utilize different types of NVCiM to improve prompt-tuning-based LLM content generation.}
  \label{fig:method}
\end{figure*}

\subsection{Past Noise Mitigation Methods}

Several strategies have been introduced to tackle the challenge of device variations in NVCiM. These methods can be separated into software and hardware-based techniques. The software-based techniques are generally developed to obtain more robust DNN models \cite{yan2023improving} and are thus not suitable for matrix-based soft prompt search.

For the hardware-software collaborative design techniques, the write-verify procedure \cite{yao2020fully} is one of the most commonly used approaches during programming. Initially, an NVM device is programmed to a set state via a designated pulse pattern. Subsequent to this, the device's value is verified to ascertain if its conductance aligns with a stipulated range of the desired value, essentially assessing its accuracy. 
% If discrepancies arise, a supplemental update pulse is initiated to reset the device conductance nearer to the target. This loop persists until the disparity between the programmed device value and the target value diminishes to a satisfactory margin, typically taking a handful of cycles. 
In this work, we take the co-design approach to design our soft prompt search algorithm based on the hardware features to ensure our framework can take advantage of NVCiM without suffering its noise impact.



==> 3_proposed_v0.tex <==
% \begin{figure*}[t!]
%   \centering
%   \includegraphics[trim=0 395 290 0, clip, width=1.\linewidth]{figures/method_Long.pdf}
%   \caption{Overview of our proposed NV\textbf{C}iM-based \textbf{P}rompt Tuning framework (\textbf{CP-tuning}). By co-design, it can utilize different types of NVCiM to improve prompt-tuning-based LLM content generation.}
%   \label{fig:method}
% \end{figure*}

% \begin{figure}[t!]
%   \centering
%   \includegraphics[trim=0 315 550 0, clip, width=1.\linewidth]{figures/method.pdf}
%   \caption{Overview of our proposed NV\textbf{C}iM-based \textbf{P}rompt Tuning framework (\textbf{CP-tuning}). By co-design, it can utilize different types of NVCiM to improve prompt-tuning-based LLM content generation.}
%   \label{fig:method}
% \end{figure}


\subsection{Framework Overview}

\rqin{Prof Xiong: describe more about our workflow, about how our prompt tuning can be different from others. Also we might need the shorter the rest of methods so we can have more space to talk about our method in high level}

As shown in Figure ~\ref{fig:method}, our proposed framework, NV\textbf{C}iM-based \textbf{P}rompt Tuning (\textbf{CP-Tuning}), consists of three parts. First, we apply the data selection method to reduce the training data samples. This data selection part can be largely effective for devices with low computational power. It conducts the representative user input embeddings. In the second part, these input embeddings will be used to train the soft prompt based on the prompt tuning method. In addition, the NVM noises are designed to inject the prompt tuning process to increase the model noise resilience towards NVM. In the third part, we introduce a retrieval algorithm to work with NVCiM, allowing us to find the appropriate trained soft prompt, which is used on the prompt tuning LLM to boost its content generation abilities. 


\subsection{Representative Selection}

In the context of user-generated data streams, it is highly probable that many samples are correlated or belong to the same domain. For such data, a single soft prompt can be shared across multiple samples. Given the constrained data buffer in our framework, the soft prompt derived from the most representative sample in a significant domain can be leveraged to enhance the Large Language Model (LLM) performance on other data within this domain. This approach significantly reduces the prompt tuning workload, which is crucial for edge devices with limited computational resources.

To identify the most representative sample, we employ a two-step process utilizing k-means clustering and cosine similarity. Given a data buffer of size $b\_s$, we first apply the k-means algorithm to group samples with similar semantic representations. The number of clusters, $n\_c$, is determined adaptively using Equation (2), which ensures a logarithmic growth from $n\_{\min}$ to $n\_{\max}$ as $b\_s$ increases beyond the base threshold $b\_0$. After clustering, we identify the largest cluster $C^*$, representing the most significant domain in the buffer. Within $C^*$, we then select the representative sample $e^*$ based on its cosine similarity to the cluster center $\mu(C^*)$, as defined in Equation (1). 

This methodology, as shown in the blue block in Figure ~\ref{fig:method}, allows us to efficiently identify a single representative sample that can be used for prompt tuning, thereby optimizing performance on edge devices with limited resources.

{\scriptsize
\begin{equation}
\begin{split}
    e^* &= \underset{e \in C^*}{\text{argmin}} \cos(e, \mu(C^*)), \quad \text{where} \\
    C^* &= \underset{C_i \in \{C_1,\ldots,C_{n_c}\}}{\text{argmax}} |C_i|, \quad \{C_1,\ldots,C_{n_c}\} = \text{k-means}(E, n_c)
\end{split}
\end{equation}
}

where $e^*$ is the most representative sample, $C^*$ is the largest cluster, $E$ is the set of all sample embeddings, $n_c$ is the number of clusters, and $\mu(C^*)$ is the center of the largest cluster. This formula selects the sample with the highest cosine similarity to the center of the largest cluster obtained from k-means clustering.


{\scriptsize
\begin{equation}
n_c = \min(\max(\lfloor n_{\min} + s \cdot \log_2(b_s/b_0) \rfloor, n_{\min}), n_{\max})
\end{equation}
}

where $n_c$ is the number of clusters, $b_s$ is the buffer size, $b_0$ is the base threshold (default: 20), $s$ is the scale factor (default: 1.5), $n_{\min}$ and $n_{\max}$ are the minimum (2) and maximum (10) number of clusters, respectively. This adaptive formula calculates the number of clusters based on the current buffer size, ensuring logarithmic growth from $n_{\min}$ to $n_{\max}$ as $b_s$ increases beyond $b_0$.

\subsection{Noise-adaptable prompt tuning}

Building upon our data selection method that identifies a representative input embedding, we now focus on training a soft prompt that enhances the LLM's content generation capabilities. In our framework, the trained soft prompt is stored in NVM for future use. However, due to inherent device variations in NVM, errors are anticipated when writing soft prompts. To address this challenge, we introduce a noise-adaptable training method that simulates device variations during the training process. This approach allows the model to account for potential NVM-induced errors, making it more robust and adaptable to various NVM designs in NVCiM.

Our noise-adaptable prompt tuning process begins with the initialization of a random soft prompt, which is then concatenated with the input embedding in the prompt encoder. This concatenated representation undergoes forward and backward passes through the LLM to calculate gradients and update the soft prompt. Crucially, we inject simulated device variation noise into the soft prompt during this process. The noise injection is governed by Equation (4), where the noise magnitude depends on the normalized value of each soft prompt element $\hat{S}_{ij}$. The noise follows a Gaussian distribution with zero mean and variance determined by the global noise parameter $\sigma$ and specific noise factors $f_1, f_2, f_3,$ and $f_4$. Finally, the noise is applied to the original soft prompt, scaled by the maximum absolute value of $S$ to maintain relative magnitude. This noise-aware training approach ensures that the resulting soft prompt is inherently robust to the device variations expected during NVM storage and retrieval.




{\scriptsize
\begin{equation}
\begin{gathered}
S' = S + N \cdot \max(|S|), \quad \hat{S} = \frac{S}{\max(|S|)} \\[-1ex]
N_{ij} = \begin{cases} 
\mathcal{N}(0, (\sigma f_1)^2) & \text{if } |\hat{S}_{ij}| > 0.75 \\[-0.5ex]
\mathcal{N}(0, (\sigma f_2)^2) & \text{if } 0.5 \leq |\hat{S}_{ij}| \leq 0.75 \\[-0.5ex]
\mathcal{N}(0, (\sigma f_3)^2) & \text{if } 0.25 \leq |\hat{S}_{ij}| < 0.5 \\[-0.5ex]
\mathcal{N}(0, (\sigma f_4)^2) & \text{if } |\hat{S}_{ij}| < 0.25
\end{cases}
\end{gathered}
\end{equation}
}

\noindent where $S'$ is the noise-injected soft prompt, $S$ is the original soft prompt, $N$ is the injected noise, $\hat{S}$ is the normalized soft prompt, $\mathcal{N}(0, \sigma^2)$ denotes a Gaussian distribution with mean 0 and variance $\sigma^2$, $\sigma$ is the gaussian\_noise\_sigma, and $f_1, f_2, f_3, f_4$ are noise factors for different intervals.

% \begin{equation}
% S' = S + N
% \end{equation}
% where $S'$ is the soft prompt after noise injection, $S$ is the original soft prompt, and $N$ is the injected noise.

% \begin{equation}
% N_{ij} = \begin{cases} 
% \mathcal{N}(0, (\sigma f_1)^2) & \text{if } |\hat{S}_{ij}| > 0.75 \\
% \mathcal{N}(0, (\sigma f_2)^2) & \text{if } 0.5 \leq |\hat{S}_{ij}| \leq 0.75 \\
% \mathcal{N}(0, (\sigma f_3)^2) & \text{if } 0.25 \leq |\hat{S}_{ij}| < 0.5 \\
% \mathcal{N}(0, (\sigma f_4)^2) & \text{if } |\hat{S}_{ij}| < 0.25
% \end{cases}
% \end{equation}
% where $\hat{S}_{ij}$ is the element of the normalized soft prompt, $\mathcal{N}(0, \sigma^2)$ denotes a Gaussian distribution with mean 0 and variance $\sigma^2$, $\sigma$ is the gaussian\_noise\_sigma, and $f_1, f_2, f_3, f_4$ are noise\_factor\_1, noise\_factor\_2, noise\_factor\_3, noise\_factor\_4 respectively.

% \begin{equation}
% \hat{S} = \frac{S}{\max(|S|)}
% \end{equation}
% where $\hat{S}$ is the normalized soft prompt.

% \begin{equation}
% S' = S + N \cdot \max(|S|)
% \end{equation}

\dcheng{delete this paragraph} This formula describes the noise injection process, including different noise intensities for different intervals and the normalization step. The noise is scaled by the maximum absolute value of the original soft prompt to maintain the relative magnitude of the noise with respect to the prompt.



\subsection{On NVM: maintain encoded soft prompt and heuristic retrieval}
% \rqin{"Should we use other words instead of compress? Since this is not our main contribution, and we want to avoid the reviewers pay too much attentions on compression, given the fact that compress is a popular topic."}

In the previous two parts, our framework can obtain the noise-adaptable soft prompts from representative data samples. The next step is to store and retrieve these soft prompts based on the NVCiM. To achieve that, we employ a pre-trained autoencoder, where the encoder can encode the soft prompts into NVM-friendly sizes and the decoder can restore the encoded soft prompts to be compatible with the LLM. In addition, we introduce a heuristic search algorithm to retrieve the appropriate soft prompt corresponding to the user input.

\subsubsection{Autoencoder to encode and restore the soft prompts}
% \rqin{Why not also use the autoencoder for noise canceling? It is hard to obtain the accurate noise for every distinct device. This paragraph of explanation should correspond to the previous explanation of using noise-mitigation over noise-cancellation.}

Due to the NVM design, the input embeddings and soft prompts usually need to be reshaped and 
encoded to better fit with NVM's memory arrays. \rqin{For example, the FeFET memory array with 128 bits <might need some help from EE side, this is shown in Figure $<$figure from Prof Ni]$>$.} For the original soft prompt, its shape normally consists of the size of virtual tokens and the dimension of embedding, with the precision of \textit{FP32}. Given the virtual token of 10 with the embedding dimension of 2048 under the embedding layer of Gemma-2, the normal soft prompt can take 5120 \rqin{FeFET memory arrays with 128 bits, which is burdensome}. When employing an autoencoder, the soft prompt embedding dimension can be 
encoded down to 48 with \textit{FP16}, where \rqin{only 60 arrays are tokens given the same FeFET-based NVM}. In our framework, as shown in Figure ~\ref{fig:method}, the autoencoder is pre-trained on certain user-generated data and decomposed into an encoder and a decoder to collaborate with our heuristic retrieval algorithm, the retrieved soft prompt will go through the decoder to restore its original shape, which can work with the trained LLM. The autoencoder allows us to map the trained soft prompts into various NVM devices. ~\ref{fig:method}, 

For on-chip computation, we employ the crossbar structure to accelerate the MAC operation.  Before the MAC operation, input embedding values are mapped to the appropriate voltage range through DAC. Soft prompts are mapped into the crossbar in advance. Due to the accuracy limitation of NVM, we use four parallel FeFETs as a cell to represent the Int16 prompt value. Four FeFETs are connected to the same word line, when input embedding voltage is applied to the word line, four FeFETs realize the same voltage. FeFET 0 corresponds to the smallest weight \(2^{0}\) , FeFET 1 corresponds to the weight \(2^{4}\), FeFET 2 corresponds to the weight \(2^{8}\) and FeFET 3 corresponds to the largest weight \(2^{12}\). The final output currents are transmitted through the respective bit lines, after TIA and ADC, the signals are converted back into digital signals. A complete int16 computation result is achieved after the bit shifter and adder.
\begin{figure}[t!]
  \centering
  \includegraphics[trim=0 245 290 0, clip, width=1.\linewidth]{figures/pengyu_figure.pdf}
  \caption{\rqin{CiM chip architecture }}
  \label{fig:circuit}
\end{figure}

\subsubsection{Heuristic algorithm to effectively retrieve the appropriate soft prompt}

\input{tables/exp_main}

\rqin{"I will leave this part here for now. Once I have the figure from Professor Ni, I will use that figure and the method overview figure to explain the heuristic algorithm."}

This heuristic algorithm is based on General Matrix Multiplication (GEMM) under the CiM architecture.

{\scriptsize
\begin{equation}
p^* = \underset{p \in P}{\text{argmax}} \text{ WMCS}(e, p)
\end{equation}
}


where $p^*$ is the most similar soft prompt, $P$ is the set of all soft prompts, $e$ is the input embedding, and WMCS is the Weighted Multi-Scale Cosine Similarity function defined as:

{\scriptsize
\begin{equation}
\text{WMCS}(e, p) = \frac{\sum_{i=1}^{|S|} w_i \cdot \cos(\text{Pool}_i(e), \text{Pool}i(p))}{\sum{i=1}^{|S|} w_i}
\end{equation}
}
Here, $S$ is the set of scales, $w_i$ is the weight for scale $i$, and $\text{Pool}_i$ is the average pooling operation with scale $i$. The cosine similarity $\cos$ is defined as:

{\scriptsize
\begin{equation}
\cos(a, b) = \frac{a \cdot b}{|a| |b|}
\end{equation}
}
The pooling operation $\text{Pool}_i$ is defined as:

{\scriptsize
\begin{equation}
\text{Pool}i(x) = \frac{1}{i} \sum{j=1}^{i} x_{k:k+i}, \quad \text{for } k = 1, 1+i, 1+2i, \ldots
\end{equation}
}
where $x$ is either $e$ or $p$, and $i$ is the scale factor.
By default, the scales $S = {1, 2, 4}$ and the corresponding weights $W = {1, 0.8, 0.6}$. This method calculates the cosine similarity between the input embedding and each soft prompt at multiple scales, applies weights to these similarities, and then selects the soft prompt with the highest weighted average similarity.
This approach allows for capturing similarities at different granularities:
\begin{itemize}
\item Scale 1 captures fine-grained, token-level similarities
\item Scale 2 captures similarities between pairs of adjacent tokens
\item Scale 4 captures broader, phrase-level similarities
\end{itemize}
The weighted average ensures that while all scales contribute to the final similarity score, fine-grained similarities (lower scales) have a higher impact than broader similarities (higher scales).










==> tables/prelim.tex <==
% \begin{table}[t!]
% \centering
% % \tiny
% \fontsize{5.5pt}{6pt}\selectfont
% \setlength{\tabcolsep}{1.8pt} % Reduced column padding to fit more columns
% \renewcommand{\arraystretch}{1.2}
% \begin{tabularx}{\columnwidth}{c|cccc|cccc|cccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c|}{\textbf{Gemma-2B}} & \multicolumn{4}{c|}{\textbf{Mistral-7B-GPTQ}} & \multicolumn{4}{c}{\textbf{Phi-2}} \\  
%  & \textbf{Vanilla} & \textbf{DEPT} & \textbf{P-t* v2} & \textbf{Single} & \textbf{Vanilla} & \textbf{DEPT} & \textbf{P-t* v2} & \textbf{Single} & \textbf{Vanilla} & \textbf{DEPT} & \textbf{P-t* v2} & \textbf{Single} \\ 
% \hline
% LaMP-1 & 0.324 & 0.392 & 0.575 & 0.735 & 0.343 & 0.255 & 0.425 & 0.529 & 0.294 & 0.324 & 0.455 & 0.755 \\
% LaMP-2 & 0.045 & 0.031 & 0.215 & 0.370 & 0.085 & 0.014 & 0.098 & 0.205 & 0.050 & 0.067 & 0.205 & 0.290 \\
% LaMP-3 & 0.392 & 0.098 & 0.590 & 0.882 & 0.363 & 0.098 & 0.354 & 0.569 & 0.461 & 0.049 & 0.667 & 0.755 \\
% LaMP-5 & 0.147 & 0.063 & 0.156 & 0.234 & 0.168 & 0.125 & 0.142 & 0.173 & 0.154 & 0.069 & 0.142 & 0.202 \\
% LaMP-7 & 0.045 & 0.066 & 0.113 & 0.240 & 0.217 & 0.170 & 0.104 & 0.198 & 0.186 & 0.231 & 0.179 & 0.254 \\ 
% \hline
% \end{tabularx}
% \caption{Performance comparisons of three edge LLMs across five datasets on three prompt tuning methods: \textbf{Vanilla} \cite{lester2021power}, \textbf{DEPT} \cite{shi2023dept}, and \textbf{P-tuning v2} (P-t* v2) \cite{liu2021p}, with the case where optimal soft prompt can be found (\textbf{Single})}
% \label{tab:one4all}
% \end{table}

\begin{table}[t!]
\centering
% \fontsize{6pt}{7pt}\selectfont
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\columnwidth}{c|cccc|cccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c|}{\textbf{Gemma-2B}} & \multicolumn{4}{c}{\textbf{Phi-2}} \\  
 & \textbf{Vanilla} & \textbf{DEPT} & \textbf{P-t* v2} & \textbf{Single} & \textbf{Vanilla} & \textbf{DEPT} & \textbf{P-t* v2} & \textbf{Single} \\ 
\hline
LaMP-1 & 0.324 & 0.392 & 0.575 & 0.735 & 0.294 & 0.324 & 0.455 & 0.755 \\
LaMP-2 & 0.045 & 0.031 & 0.215 & 0.370 & 0.050 & 0.067 & 0.205 & 0.290 \\
LaMP-3 & 0.392 & 0.098 & 0.590 & 0.882 & 0.461 & 0.049 & 0.667 & 0.755 \\
LaMP-5 & 0.147 & 0.063 & 0.156 & 0.234 & 0.154 & 0.069 & 0.142 & 0.202 \\
LaMP-7 & 0.045 & 0.066 & 0.113 & 0.240 & 0.186 & 0.231 & 0.179 & 0.254 \\ 
\hline
\end{tabularx}
\caption{Performance comparisons of two edge LLMs across five datasets on three prompt tuning methods: \textbf{Vanilla} \cite{lester2021power}, \textbf{DEPT} \cite{shi2023dept}, and \textbf{P-tuning v2} (P-t* v2) \cite{liu2021p}, with the case where optimal soft prompt can be found (\textbf{Single})}
\label{tab:one4all}
\end{table}





